Recent Advances in Hierarchical Multi-label Text Classification: A Survey

Hierarchical multi-label text classification aims to classify the input text into multiple labels, among which the labels are structured and hierarchical. It is a vital task in many real world applications, e.g. scientific literature archiving. In this paper, we survey the recent progress of hierarchical multi-label text classification, including the open sourced data sets, the main methods, evaluation metrics, learning strategies and the current challenges. A few future research directions are also listed for community to further improve this field.

==> content/sec1_old.tex <==
\section{Introduction}
As a fundamental problem in natural language processing, multi-label text classification means assigning documents to multiple labels. However, people gradually notice that the hierarchical relationships between different labels is also an extra important information which can help classify. Thus Hierarchical Multi-label Text Classification refers to that texts are associated with multiple class labels which are organized in a structured label hierarchy. Currently, there are many and complex models for hierarchical multi label tasks, and few literature has summarized such topics. Therefore, we have conducted a survey of the literature on hierarchical multi-label text classification in recent years. This survey is mainly composed of six parts. The second part introduces the background and development status of hierarchical multi-label tasks. The third part summarizes the data set used for hierarchical multi-label classification. The fourth part mainly discusses the models and methods used for hierarchical multi-label text classification in the literature we have investigated, and divides these models into four major categories. The fifth part shows some learning strategies used in this task. The sixth part mainly summarizes the evaluation indicators. The seventh part proposes some challenges for the current hierarchical multi-label classification task. The last part is the conclusions drawn and suggestions for future work.

==> content/sec2.tex <==
\section{Background}
With the rapid development of the information age, the number of articles is increasing at an explosive rate. Manual tagging of relevant articles has become very time-consuming, and there is a certain impact of subjective consciousness in manual tagging. Therefore, text classification has more practical significance. With the progress of scientific research on text classification, people gradually notice that the same article may have different labels, However, there may be some associations between different tags. For example, some tags can be classified as child tags or parent tags of other tags in some scenarios. Specifically, a news article can be classified into three categories: "sports", "basketball" and "warrior", of which "basketball" is a subclass of "sports" and "warrior" is a subclass of "basketball". The relationship between the class labels is described as hierarchical relationship. The text classification task with this relationship is called hierarchical multi-label text classification task. In mathematics, hierarchical multi-label classification can be defined as a function:
$
f: X \rightarrow Y^*
$
where $X$ is the sample space and $Y^*$ is the power set of all possible label sets. Each element in Y * is an ordered tag sequence $(y_1, y_2,..., y_k)$, representing the hierarchical path from the root node to the leaf node. For example, (sports, basketball, warrior) is an effective tag sequence. The goal of hierarchical multi-label classification is to learn a function $f$, so that for any given sample $x \in X$, $f (x)$ can output one or more tag sequences most relevant to $x$.\\
The hierarchical multi-label classification task is mainly to calculate the dependency relationship between labels and find labels at different levels in a large number of label data sets. At present, there are many researches in this field. The overall idea is to obtain the data set, preprocess the text, and then put it into a specific classifier through different models to achieve the output of different categories of text labels. Researchers focus on creating good models to learn the mapping of instances to tags and complete classification. Multi-level classification will use graph relations to separate labels and document metadata, which can make the whole process faster. \\
\\
In 2014, Yoon Kim first applied the CNN structure to the text classification task\cite{kim-2014-convolutional}, followed by the TextRNN model, followed by the hierarchical attention network model HAN \cite{yang-etal-2016-hierarchical}, and added the attention mechanism to TextRNN for the first time, using a hierarchical structure to represent a text, which is well interpretable. In order to solve the label masking problem, the BERT model \cite{2018arXiv181004805D}for sequence generation was proposed. In addition, RNN network is also very popular. RNN-GRU uses GRU to make the original model have a better classification starting point. At the same time, there are many label classification methods based on graph, tree and other data structures. Although the ultimate purpose of hierarchical multi-label classification is the same as that of traditional text multi-label classification, because it introduces the hierarchical structure of labels, multi-label text classification also faces problems such as inaccurate labels and unclear definitions of dependencies between labels. In this article, we will summarize different models and methods in hierarchical multi-label text classification on different dimensions, and we will also analyze the challenges in future work.

==> content/sec2_old.tex <==
\section{Background}
With the rapid development of the information age, the number of articles is increasing at an explosive rate. Manual tagging of relevant articles has become very time-consuming, and there is a certain impact of subjective consciousness in manual tagging. Therefore, text classification has more practical significance. With the progress of scientific research on text classification, people gradually notice that the same article may have different labels, However, there may be some associations between different tags. For example, some tags can be classified as child tags or parent tags of other tags in some scenarios. Specifically, a news article can be classified into three categories: "sports", "basketball" and "warrior", of which "basketball" is a subclass of "sports" and "warrior" is a subclass of "basketball". The relationship between the class labels is described as hierarchical relationship. The text classification task with this relationship is called hierarchical multi-label text classification task. In mathematics, hierarchical multi-label classification can be defined as a function:
$
f: X \rightarrow Y^*
$
where $X$ is the sample space and $Y^*$ is the power set of all possible label sets. Each element in Y * is an ordered tag sequence $(y_1, y_2,..., y_k)$, representing the hierarchical path from the root node to the leaf node. For example, (sports, basketball, warrior) is an effective tag sequence. The goal of hierarchical multi-label classification is to learn a function $f$, so that for any given sample $x \in X$, $f (x)$ can output one or more tag sequences most relevant to $x$.\\
The hierarchical multi-label classification task is mainly to calculate the dependency relationship between labels and find labels at different levels in a large number of label data sets. At present, there are many researches in this field. The overall idea is to obtain the data set, preprocess the text, and then put it into a specific classifier through different models to achieve the output of different categories of text labels. Researchers focus on creating good models to learn the mapping of instances to tags and complete classification. Multi-level classification will use graph relations to separate labels and document metadata, which can make the whole process faster. \\
\\
In 2014, Yoon Kim first applied the CNN structure to the text classification task\cite{kim-2014-convolutional}, followed by the TextRNN model, followed by the hierarchical attention network model HAN \cite{yang-etal-2016-hierarchical}, and added the attention mechanism to TextRNN for the first time, using a hierarchical structure to represent a text, which is well interpretable. In order to solve the label masking problem, the BERT model \cite{2018arXiv181004805D}for sequence generation was proposed. In addition, RNN network is also very popular. RNN-GRU uses GRU to make the original model have a better classification starting point. At the same time, there are many label classification methods based on graph, tree and other data structures. Although the ultimate purpose of hierarchical multi-label classification is the same as that of traditional text multi-label classification, because it introduces the hierarchical structure of labels, multi-label text classification also faces problems such as inaccurate labels and unclear definitions of dependencies between labels. In this article, we will summarize different models and methods in hierarchical multi-label text classification on different dimensions, and we will also analyze the challenges in future work.

==> content/sec3_old.tex <==
\section{Data sets}
In this section, we will introduce the common hierarchical multi-label classification data sets and divide them into three categories: emotion categories, articles categories, and topic categories. We count 17 commonly used data sets and analyze their source, content, hierarchy and other information. Among them, there are four emotion data sets, 7  article datasets and 6 topic datasets.
\subsection{Emotion  data sets}
Such data sets mainly include user emotion labels,Using for performing the emotion-label classification,being common in a variety of food reviews, film reviews and other data sets.\\
\\
\textbf{YELP} The YELP data set is sourced from the US restaurant review website and consists of 60,000 merchants, 8.63 million comments and 200,000 images. This data set shows the different scores of users for the store, which is divided into two sub-data sets: YELP-2 and YELP-5. User reviews of YELP-2 mainly use positive and negative emotion labels, while YELP-5 reviews have five different scores.\\
\\
\textbf{Amazon Product Reviews} This dataset contains a large number of user product reviews of Amazon, with about 8 million reviews. Emotional labels are also divided into binary categories and multi-class categories, just like YELP. Its common sub-datasets include Amazon-670k, Amazon-3m, etc.\\
\\
\textbf{IMBD} IMBD is a binary sentiment classification dataset containing both positive and negative ratings. It has 50k samples and the testing set and the training set both have 25k of them. All data are obtained from film reviews on the IMBD website.

\begin{table}
\centering
\caption{Emotional data sets}\label{tab1}
\begin{tabular}{|c|c|c|c|}
\hline
Name &  Field & Number of categories & Level depth\\
\hline
YELP & Dining reviews & 539 & -\\
Amazon 670k & Product reviews & 670091 & 9\\
Amazon 3M & Product reviews & 2812281 & -\\
IMBD & movie reviews & - & -\\
\hline
\end{tabular}
\end{table}


\subsection{Article classification data sets}
These data sets have information on a large number of different articles that may originate from the same websites or journals. The content of the article may involve various aspects.\\
\\
\textbf{WOS}  The WOS dataset contains web of science articles, with 134 catalogues and 46,985 instances, covering all aspects. This data set is a common data set for hierarchical multi-label classification. There are three categories: WOS-5736, WOS-11967, WOS-46985. WOS-5736 and WOS-11967 are subsets of WOS-46985.\\
\\
\textbf{Arxiv}  The Arxiv dataset has about 1.7million articles, divided into 14 different features, such as authors, titles et al. It is divided into 62,055 subcategories according to different disciplines, which basically includes most of the papers on the arxiv website.\\
\\
\textbf{Pubmed} The Pubmed dataset is a dataset about biomedicine and has its own retrieval function. The data set contains approximately 20,000 instances, and all of them are scientific research papers on diabetes. Each instance in the dataset is represented by a weighted word vector. \\
\\
\textbf{Reuters Corpora}  This data set is a collection of Reuters news and articles and have two versions. RCV1 is modified on the Reuters-21578 dataset and has 8 million instances in English. RCV2 has nearly 5 million instances in 13 different languages.Both are very commonly used text classification data sets.\\
\\
\textbf{NYTimes}  This dataset contains 1.8 million articles from New York Times during 1987-2007. It is a very large dataset,which widely used in NLP studies such as document categorization, entity extraction, etc.
\begin{table}
\centering
\caption{Emotional data sets}\label{tab1}
\begin{tabular}{|c|c|c|c|}
\hline
Name &  Field & Number of categories & Level depth\\
\hline
WOS  & Academic articles & 141 & 2\\
WOS-11967 & Academic articles & 40 &2\\
Arxiv & Academic issues & -& -\\
Pubmed & Biomedical articles & 17693 & 15\\
Reuters  & News & 101 & 3\\
RCV1 &Reuters news &103 &6\\
NYTimes & News & 2318 & 10\\
\hline
\end{tabular}
\end{table}
\subsection{Topic classification data sets}
Each data set is mainly about a certain topic.The data set includes information about one specific topic,such as patents,book advertising,bookmarks,etc.\\
\\
\textbf{HUPC}  This dataset covers 4.5 million patent documents in English. The patents come from the USPTO website which all applied in 2004-2018. This dataset provides the structured metadata for each application in order to be better utilized by researchers.\\
\\
\textbf{BGC-EN}  Blurb Genre Collection (BGC) is a data set of book advertising descriptions, and each bulbar is divided into one or several categories. This data set consists of 91,892 instances, including the book’s title, the author, url, ISBN, etc.\\
\\
\textbf{WIPO}  This dataset is a very typical patent dataset, similar to HUPC. This dataset contains 74,650 samples from the World Intellectual Property Organization (WIPO). It contains the ID, author, class and other information of the patent, of which 45324 samples are used for the training set and 28926 are used for the test set.
\\
\\
\textbf{DBpedia} This is a very common data set in NLP research. The information in this data set is extracted from Wikipedia. DBpedia is updated monthly to add or delete some data and adjust the categories. It has a lot of sub-datasets, for example: DBpedia Ontology Dataset, which has 630k instances; Dataset 3.8, which has 3.77 million samples.\\
\\
\textbf{Delicious}  Delicious is a social platform for sharing and discovering bookmarks. Data for Delicious dataset comes from this site and contains the users’ ID and friendship between the users. In the two available CSV files, there are 103144 nodes and 1419519 edges.\\
\\
\textbf{Enron} The dataset, collected by the CALO project, contains data from approximately 150 users. There are 0.5M samples in the dataset, divided into 56 labels.\\
\begin{table}
\centering
\caption{Emotional data sets}\label{tab1}
\begin{tabular}{|c|c|c|c|}
\hline
Name &  Field & Number of categories & Level depth\\
\hline
HUPC  & Patent information & - & -\\
BGC-EN  & books’ introduction & 146 & 4\\
WIPO-alpha & Patent information &5229 &4\\
DBpedia & Wikipedia data & - & -\\
Delicious & User Information & 983 & -\\Enron & Email information & 56 & 3\\
\hline
\end{tabular}
\end{table}

==> content/sec4_old.tex <==
\section{Methodology}
\subsection{tree}
In this method, labels are organized into a tree structure, and predict the labels of each sample by recursively processing the relationship between child nodes and parent nodes. The tree models make the structure very clear, but most of them are early models. Thus the accuracy may not very high. \\
\\
\textbf{AttentionXML} 
 AttentionXML was published by Ronghui You in 2019\cite{2018arXiv181101727Y}, which used attention model and a PLT to improve performance.This model mainly wants to solve the defects of the BOW method and XML-CNN, such as the lack of flexibility and the capture of label information.The model does two things:(1)build a shallow and wide PLT.Each leaf on the PLT represents a label  and the PLT divides the label continuously recursively into two smaller clusters.Complete initialization by the sum of the bow features of the normalized text and then compress this tree.This model does not use deep label trees, because large trees or large clusters create problems that tail labels are not distinguishable, and there may be propagating and cumulative errors.(2) Build a five-layer attention model.The PLT at each level trains deep model to calculate context vectors for each label,in order to capture the most relevant labels.\\
 
This model has one problem, that is, the label awareness is not strong enough. The model does not consider the level correlation between labels, so may be it can be further modeled on the label information.\\
\\
\textbf{FastXML} FastXML\cite{10.1145/2623330.2623651} is also a model based tree. Its characteristic is fast. FastXML draws on multi-label random forest (MLRF) algorithm and sublinear ranking label (LPSR) partition algorithm, but it is faster than the most advanced MLRF and LPSR. The root node contains the whole label set. Whether the label should be assigned to the left child node or the right child node depends on a algorithm named node partitioning formulation. Like this, recurse until you reach the leaf node with only a few labels. The purpose of training is to fit a reasonable tree structure. When predicting, a data point can be passed along the tree until it reaches the leaf node. Then the classifier can be applied to these leaf nodes. This algorithm is local and cannot measure the whole situation. Optimizing global measurement may be expensive, because global measurement in the tree requires joint learning of all nodes.\\
\\
\textbf{HyperIM}  Hyperbolic representation capability\cite{DBLP:journals/corr/abs-1905-10802} is also a way to indicate the label hierachy. The primary reason is that the tree-like structure of hyperbolic space is well-suited for modeling symbolic data with hierarchical structures, which are often complex. Thus HyperIM is proposed which embeds both document words and labels jointly in the hyperbolic space to preserve their latent structures. HyperIM uses the text sequence of a document to measure the similarities between words and labels. To do this, it calculates the geodesic distance between words and labels that are jointly embedded in the Poincaré ball. After obtaining the word-label similarity scores, HyperIM aggregates them to generate label-aware document representations. These representations are then used to predict the probability of each label. The innovation of this method is that it can connect words in documents and labels, and use the most relevant part of documents to build the representations of the article, so as to improve the accuracy of classification. \\
\\
\textbf{Using CSSA with KDE} In this issue\cite{10.5555/3104482.3104485}, the authors creatively combined KDE with the CSSA algorithm.The problem was converted to a single-label calculation problem with kernel dependency estimation (KDE)and generalized CSSA is used to find the optimal subgraph in DAG to construct multiple labels with consistent hierarchical structure.KDE algorithm is to project labels into each dimension, learn them separately, get multiple predictions, and then map them into the original label space. This is the problem transformation method, which is more flexible than the adaptive method.The author improved the CSSA algorithm: (1) for the tree: the key is to merge the nodes. If the parent node is selected,then select it as well; if not, combine the parent node with the parent node.(2) For DAG: the CSSAG algorithm is proposed: when the label is inconsistent with the DAG, and the supernode is merged with the unassigned minimum parent node. That is, earlier supernodes are used first. However, for DAG of OR property, replication of subnodes is required before merging.
The advantage of this algorithm is that the labels can be fully learned using the whole dataset, and that the labels' insufficient learning will not happen.\\
\\\textbf{Hierarchically Regularized Deep Graph-CNN}  HR-DGCNN\cite{Peng2018LargeScaleHT} is a model proposed for discontinuous semantics and long-distance semantics. The model is mainly divided into three parts, input, convolution layer and output. The paper on the input layer has done a very interesting treatment. The input of the text data in the paper is to convert the text into a graph by using the co-occurrence of words. Then the nodes in the graph are sorted and divided into different sub-graphs (using the degree of nodes and the number of times words appear in the document to determine the sorting order) and the sub-graphs are regularized. Finally, word embedding is performed using the trained word2vec model. This results in a good word embedding input. The paper does not differ from the basic CNN model in the processing of the convolutional layer and the output layer, so we will not discuss it. But in the fully connected layer, the paper has done recursive regularization in the fully connected layer of the last layer. The so-called recursive regularization makes labels that are close in the hierarchy have similar parameters. At the same time, the paper also mentioned a method of recursive hierarchical segmentation, mainly to solve the large-scale hierarchical multi-label classification problem.\\ 
\\
\textbf{Bonsai Algorithm} Bonsai\cite{2019arXiv190408249K} is an algorithm proposed to solve extreme multi-label classification problems. The main innovation of this method is to build a shallow tree structure. For data input, the paper summarizes the previous three methods of generating label representations, namely input space representation, output space representation, and input-output space joint representation. After the tag representation is generated, the K-Means clustering algorithm is used to partition the resulting tag representation, and a shallow tree structure of related tags is generated through this clustering method. The paper divides all the labels into K sets through the clustering method, then establishes the root node, and links the root node with the separated classes (at this time, the K clusters will become the child nodes of the root node). Then perform the same clustering algorithm for each child node, and then continue to build new nodes until the nodes of the subtree are greater than the specified maximum depth value or the number of associated labels in the subtree is not greater than K. In the paper, in order to avoid propagation errors in deep tree cascades, a larger K value (k greater than or equal to 100) is set. In the prediction stage of the model, the paper adopts the one-vs-rest method for prediction. By using the shallow tree structure obtained earlier, set a linear classifier for each node. For nodes that are not leaf nodes, according to the predicted output of each non-leaf node in the current layer, judge whether to traverse the child nodes of these nodes according to the output results (to avoid unnecessary operations). For leaf nodes, only the node itself needs to be classified.\\
\\
\textbf{summary} For the tree-based methods, their advantages are that they can use the hierarchical structure between labels more accurately and the prediction results of the model are easy to explain. The disadvantage is that there is a high requirement for tag level knowledge that needs to be acquired in advance and accurate hierarchy information is required. Besides, because it uses a relatively simple tree structure model, it is difficult to deal with the complex dependency relationship between labels, which needs to be represented by a more powerful model.

\subsection{hierarchical step by step prediction}
hierarchical step by step prediction means labels at each level are predicted independently, and the prediction of each label depends on the results of the label predictions of the previous level.\\
\\
\textbf{Capsule network}  Capsule network \cite{aly-etal-2019-hierarchical} has a good performance in the field of natural language processing, which can mainly solve the problem of information loss during pooling. Capsule network can capture the categories’ underlying structures by associating each label with one capsule. An output of a capsule is a vector, not a single scalar value used in traditional neural network, so that it can encode more information of each category. The working principle of the capsule network is that the first layers prepossess the input data. After the data prepossessing, the results will be sent to the primary capsule layer, and a vector with potential information will be output. For each classification capsule, it weights the output of all primary capsules and predict the label probability by using squashing function. The connection between layers is based on routing algorithm, which can determine the contribution of each primary capsule’s output to a classification capsule, reflecting the hierarchy of labels. The benefit of using capsule network is that articles can be encodes with more messages, but not all of this information is useful. Valid information is always hard to get. Besides, due to the use of routing algorithm, there is also a problem of slow calculation. \\
\\
\textbf{Hierarchical Transfer Learning}  HTrans\cite{banerjee-etal-2019-hierarchical}, a Hierarchical Transfer Learning approach, is proposed, which uses a Gated Recurrent Unit (GRU)-based deep learning architecture coupled with attention. Attention is applied on top of the GRU. This model combines a max-pooled and mean-pooled representation of all the GRU hidden along with attention to feed into output layer. Binary classifiers are used for prediction, which provide more flexibility than training a single multi-label classifier, and can solve the problem of imbalance distribution of label data. In HTrans, binary classifiers at lower levels in the hierarchy are initialized using parameters of the parent classifier and fine-tuned on the child category classification task. Learning rate plays a more important role in this scene, so how to find a smart way to adjusting hyper-parameter need further try and research.\\
\\
\textbf{Hierarchical Fine-Tuning} Hierarchical Fine-Tuning(HFT)\cite{shimura-etal-2018-hft} was proposed in a paper published by Kazuya Shimura in 2018. HFT is mainly to solve the poor low-level label classification results caused by the non-hierarchical planar model when performing hierarchical classification. Therefore, this paper uses CNN as the basic model (a typical non-hierarchical planar model). In the process of training the model, the parameters of the word embedding layer and the convolutional layer are mainly transferred from top to bottom, that is, the parameters of the upper layer structure are used to learn the labels of the lower layer. At the same time, in order to avoid adverse effects caused by excessive correlation gaps between distant levels, parameter fine-tuning is only performed between adjacent levels.\\
\\
\textbf{Loosely Coupled Graph Convolutional Network} Loosely coupled graph convolutional neural network (LCGCN)\cite{xu-etal-2021-hierarchical} is a GCN model, mainly to solve the over-smoothing problem caused by too many nodes or edges of the GCN graph model. LCGCN mainly consists of two parts of the graph model, one part is the core graph, which is used to extract word embeddings and category embeddings; the other part is the document-word graph, which is mainly used to capture the relationship between documents and words. At the same time, in order to make full use of the correlation between categories, this paper also proposes a new method to capture the relevant information between different levels and different categories from horizontal correlation and vertical correlation respectively. For horizontal correlation, the article defines a correlation matrix, which can be obtained through the softmax function of the singular matrix embedded in the h-th layer category obtained from the core map, and then coupled with the label to obtain the $h$ layer Relationships between horizontal categories. The paper's vertical processing is very ingenious, fully considering the information structure of the upper layer and cleverly integrating the relationship between categories into the document representation. This method mainly uses the category embedding of the current layer obtained in the core graph, and dot-multiplies it with the prediction result of the current layer, and we can obtain a new vector representation of the category. Finally, the obtained new category representation is coupled with the current document embedding to obtain a new document representation, which will be used as the document input for the next layer. The results obtained by the above two correlation methods are applied in the final loss function for gradient optimization and parameter update.\\
\\
\textbf{Coherent Hierarchical Multi-Label Classification Networks} C-HMCNN\cite{2020arXiv201010151G} model was raised by Eleonora Giunchiglia,which used networks to generates predictions consistent with the hierarchical constraints. Many neural network models produce incoherent predictions and require a  additional post-processing step to be coherent with hierarchical constraints,while C-HMCNN can achieve coherent output without additional steps.C-HMCNN uses the loss function to make the hierarchical structure of the lower layer to predict the upper layer.This model has two parts:(1)There are two bottom modules of outputs that ensure  no hierarchical conflicts occur.(2) A maximum constraint module (MCM), which has a layer of input and implements hierarchical restrictions. In MCM, the maximum constraint loss function is trained so that hierarchical constraints can be exploited.The author used 20 datasets to prove this model can improve the performance.\\
\\
\textbf{LA-HCN} LA-HCN\cite{2020arXiv200910938Z}, whose full name is Label-based Attention for Hierarchical Mutlti-label Text Classification Neural Network, also extracts important information from the text hierarchically for labels from different hierarchical levels to. The label-based attention is used to bridge the labels and document content. Unlike the features extracted from typical attention may be diluted, it can extract meaningful information corresponding to different labels to learn learning disjoint features for each hierarchical level. Level information is transferred between layers. Besides, both local and global classifiers are applied to this model to get the final result, which can prevent the fact that with only local classifiers,the wrong classification of a local classifier will spread to the next level, thus affecting the final global classification. 
\\
\\
\textbf{HMCN-(F/R)} The HMCN-(F/R)\cite{wehrmann2018hierarchical} model is a combination of the HMCN-F and HMCN-R models. The HMCN-F model is a new model constructed to coordinate local information and global information. There are mainly two ways of information transmission in the model. The first is the main flow, where information passes from the input layer through the fully connected layer to the global output layer. The output of each layer is multiplied by the output of the previous layer and the input data of the model, after a linear change, and finally through a nonlinear activation function to obtain the output of the corresponding level. The second information transmission of the HMCN-F model is the local flow, which uses the output of the main information flow to perform two consecutive transformations to obtain the local information corresponding to the hierarchical structure. Finally, the outputs obtained from the two information streams are integrated to obtain the final prediction result of the HMCN-F model. The point of HMCN-F is to make full use of local information and global information. But as the label hierarchy increases, the HMCN-F model parameters also increase. Therefore, when the hierarchy is deep, it will lead to a sharp increase in the number of model parameters. To solve this problem, HMCN-R is proposed. HMCN-R still retains the idea of extracting local information from the main information flow, but HMCN-R refers to the structure of LSTM in structure, which will greatly reduce the consumption of parameters, thus fundamentally solving the problem of HMCN-R. F-parameters increase dramatically. HMCN-(F/R) output includes hierarchical output and global output, and the corresponding loss function is also composed of local loss and global loss. Since the consistency of hierarchical classification cannot be guaranteed by minimizing local loss and global loss, Therefore, the article proposes a hierarchical penalty loss to reduce this risk, expressed as $\mathcal{L}_{H_i} = \lambda \mathop{max}\{0,Y_{in}-Y_{ip}\}^2 $ where $Y_{in}$ and $Y_{ip}$ represent the predicted scores of child nodes and parent nodes .So the final loss function can be expressed as 
$$
\mathop{min}\limits_{W}\{\mathcal{L}_L + \mathcal{L}_G + \mathcal{L}_H\} 
$$\\
\\
\textbf{Summary} The popularity of this kind of model can be observed from the abundance of pertinent documents, as it is a highly structured and high-performing approach. The advantages of this kind of model include its ability to capitalize on label correlations for enhanced model accuracy, as well as its capacity for parameter sharing across multiple tasks to optimize computing resources. However, this kind of model also presents certain disadvantages, such as its challenging training process and complex structure.
\subsection{label plus text as input, simultaneous prediction}
The hierarchical structure of the label is entered into the model structure as known information, so the hierarchical structure information of the label can be used in the prediction of the label. The modeling of label hierarchy mostly uses graph model.\\
\\
\textbf{Metadata and Label Heterogeneous Graphs}  Many methods simply use metadata semantic information or established parent-son label structure, ignoring the heterogeneous graph structure. Heterogeneous graphs\cite{ye-etal-2021-beyond} are used by  Chenchen Ye to model labels' hierarchy and their statistical dependencies. Besides,the author also consider the metadata in the documents,which still be modeled by heterogeneous graph. This paper presents two heterogeneous maps: metadata heterogeneous map and label heterogeneous map and through these two heterogeneous graphs, the topological relation of the metadata and the hierarchy and dependence of the labels can be obtained.The author built a three-layer model to analyze, with multiple transformer layer, and used MHA and FFN methods to pass the parameters layer by layer.And use the heterogeneous map conversion (HGT) to analyze the above two heterogeneous maps.HGT contains Heterogeneous
Mutual Attention(ATT), , Heterogeneous Message Passing (MSG)and Target-Specific Aggregation(AGG) to obtain the vector of metadata and labels.Then by activate the function and the linear transformation layer, get the document text vector, and finally output the result through the prediction function.\\
\\
\textbf{Hierarchy-Aware Global Model}  In this paper\cite{zhou-etal-2020-hierarchy}, the hierarchy is represented as a directed graph, which is read into the encoder,modeling labels' dependencies with structural encoders.The authors propose the HiAGM global aware model, containing the label structure encoder, the text encoder.There are two submodels:(1) HiAGM-LA: The label  features can be fused with each other, and the text and label are independently expressed and predicted by attention mechanism.(2) HiAGM-TP: Text features can be directly input into the structural encoder to participate in the feature calculation.The article also proposes two types of structure encoder for labels:(1) Bidirectional Tree-LSTM: The LSTM structure is used to encode the tree  data structure, and the two-way tree corresponds to the two directions between the parent nodes and children nodes.(2): Hierarchy-GCN: GCN calculation the adjacent nodes of one node. This model better captures the hierarchical information and more fully utilizes the interaction of text features and label features.\\
The main problems in this paper are the possible lack of a loss function to calculate the differences between the children nodes, and the lack of some commonly used baselines for the model performance comparison.\\
\\
\textbf{Summary} This kind of model inputs the hierarchical information of labels into the network as known knowledge, and some documents also use the meta data of documents as input. The advantages of this method is that it can better handle the complex dependency between tags. Besides, the model design structure is not complex, which only needs to model and represent the hierarchical structure. However, the classifier cannot make more targeted use of the hierarchical structure between labels. What's more, the prediction results of the model are difficult to explain.
\subsection{ensemble (parallel)}

Ensemble is also a great idea. Labels at each level are predicted separately. This is done in parallel. After output, predicted labels interact with each other with hierarchical structure information to get final results, like voting in prediction time. However, this method is mostly used in the industrial field and is suitable for large engineering projects, so the number of models is not large.\\
\subsubsection{one-vs-one} One-vs-one refers to having a classifier between each two categories. This looks great, but as the number of levels of labels increases, the number of classifiers increases dramatically. When there are n categories here, then the number of the classifiers will grow to $C_{n}^{2}$. Thus this method is uncommon.
\subsubsection{one-vs-all} One-vs-all means every label has a special classifier. For each classifier, each classifier treats its corresponding category as a positive example and treats the remaining categories as negative examples. In this way, the number of classifiers is greatly reduced. The paper\cite{10.1007/978-3-031-17189-5_14} uses this method. The Author proposed two modules: a shared encoding module and a task-specific module. First, the language model SciBERT was pre-trained. The vector obtained by encoding the text feed into the task-specific module, where the sub-task of classifying each tag is performed. And then a shared TextCNN layer was introduced to learn the dependency information between labels at each level. Finally, the hierarchical feature information is fused by linear transformation and the prediction result of each level is getted.



==> content/sec5_old.tex <==
\section{Learning Strategies}
\subsection{self-training} Self training is a semi supervised learning method in which a small amount of labeled data is used for initial training, and then prediction results are used to generate more training data. In hierarchical multi label classification tasks, self training can generate more training data by using the prediction results of the current model, and then use these data for the next round of training.
\subsection{semi-supervised} Semi-supervised learning is a method of using unmarked data to enhance supervised learning. In hierarchical multi label classification tasks, semi supervised learning can use unlabeled data to learn hierarchical relationships between labels, and then use these relationships in supervised learning.\\
\\
\textbf{weakly-supervised hierarchical multi-label text classification} In reality, a real situation is that there is no large number of human tagged documents to train classifiers, so approaches based on only class surface names as supervision signals are explored. Thus TaxoClass\cite{shen-etal-2021-taxoclass} is proposed. First, a pre-trained textual entailment model is used to  calculate the document-class similarity. After that, the calculated similarity is used to determine the core class of the article. Then training data extracted from document core classes is used to train a text classifier. The classifier includes a document encoder based on pre-trained BERT, a class encoder capturing class taxonomy structure, and a text matching network computing the probability of a document being tagged with each class. The class Encoder is a graph neural network to capture the hierarchical information of label. This method can train a large number of unlabeled documents, but because of the unlabeled data, the determination of the core class of the document may not be so accurate, which may affect the final accuracy. \\
\\
\subsection{data augmentation}
Data augmentation is a commonly used training strategy that can increase the diversity of training data and help models better generalize to new data. In hierarchical multi label classification tasks, data augmentation can be used to generate more training data, and can help models learn hierarchical relationships between labels by generating data related to hierarchical relationships.Data enhancement can be implemented in the following ways: Synonym Replacement, Random Insertion, Random Deletion, Random Swap, and Sentence Rearrangement. The above methods can be randomly applied to training data with a certain probability, thereby expanding the dataset and increasing the generalization ability and robustness of the model. At the same time, it is also important to note that excessive data enhancement may lead to over fitting of the model, so it is necessary to make choices based on specific tasks and data characteristics.

\subsection{label enhancement}
Label enhancement is a method of enhancing original label information through the use of external resources (such as knowledge maps, dictionaries, corpora, etc.). In hierarchical multi label classification tasks, label enhancement can help models more accurately understand and depict the relationship and semantic information between different labels, thereby improving the classification accuracy and generalization ability of the model.However, it should be noted that excessive label enhancement may introduce noise and incorrect labels, thereby reducing the performance and generalization ability of the model. Therefore, this method needs to be used appropriately. 
 

\subsection{post-processing}

==> content/sec6_old.tex <==
\section{Evaluation Metrics}

Before understanding the following evaluation indicators, we must know some of the meanings of the following expressions. For multi label classification tasks, we assume that there is a set of $D$ that is a multi label dataset consisting of $n$ samples $(x_i, Y_i)$, $1\leq i\leq n$. If $c$ is a multi label classifier, then $Z_i = c(x_i)$ is the predicted output of the corresponding $x_i$.

\subsection{label-based}
\textbf{Precision:} Accuracy is the ratio of the predicted correct labels to the total number of actual labels. The average of all instances, known as the accuracy rate. In a multi label classification task, the accuracy rate is actually the average accuracy rate of each sample, and its calculation formula is as follows:
$$
    Precision = \frac{1}{N}\sum_{i=1}^N\frac{|Y_i\cap Z_i|}{|Z_i|}
$$
\\
\textbf{Recall:} Recall rate refers to the ratio of correctly predicted labels to the total number of predicted labels, which is averaged across all instances. For each sample, the recall rate is to predict the proportion of the correct number of labels in the overall correct number of labels.
$$
    Recall = \frac{1}{N}\sum_{i=1}^N\frac{|Y_i\cap Z_i|}{|Y_i|}
$$
\\
\textbf{F1-score: }This evaluation index is actually the harmonic average of Precision and Recall, and its calculation formula is:
$$
  F1-score = \frac{1}{N}\sum_{i=1}^N\frac{2|Y_i\cap Z_i|}{|Y_i|+|Z_i|}=\frac{2\times Precision\times Recall}{Precision+Recall}  
$$
\subsection{example-based}
\textbf{Accuracy:}Accuracy refers to the accuracy of each instance, defined as the ratio of the predicted correct tags to the total number of tags for that instance (predicted and actual), which can measure how close the measures we have taken are to the true value. In the multi label classification problem, the accuracy rate actually calculates the average accuracy rate of all samples. For example, if the true label of a sample is $[0,1,1,0]$, and the prediction label is $[0,1,0,1]$, then the accuracy of the sample is $\frac{1}{1+1+1}=\frac{1}{3}$, so the global accuracy calculation formula is as follows:
$$
    Accuracy = \frac{1}{N}\sum_{i=1}^N\frac{|Y_i\cap Z_i|}{|Y_i\cup Z_i|}
$$
\\
\textbf{Hamming Loss: }This evaluation indicator is the most intuitive and easily understood one, which directly counts the number of incorrectly classified labels. Hamming Loss measures the proportion of incorrectly predicted tags in the total number of tags in all samples, and its specific calculation formula is as follows ($Y_j^{(i)}$represents the $j^{th}$ label of the $i^{th}$ sample):
$$
    Hamming\; Loss = \frac{1}{kN}\sum_{i=1}^N\sum_{j=0}^q I(Y_j^{(i)}\neq Z_j^{(i)} )
$$
\\
\textbf{Subset Accuracy:}
$$
    Subset \;Accuracy = \frac{1}{N}\sum_{i=1}^N I[Y_i=Z_i]
$$
\subsection{ranking-based}
\textbf{P@k} Full name is Precision@k. The calculation formula is similar to Precision:
$$
    P@k = \frac{1}{N}\sum_{i=1}^N \frac{|Y_i\cap Z_i|}{\min(k,|Y_i|)}
$$
\\
\textbf{AUC} The full name of AUC is Area under the curve. AUC is defined as the area enclosed by the coordinate axis under the ROC curve. It represents the ability of the model to correctly distinguish between positive and negative samples, with a value range of 0.5 to 1. The higher the AUC value, the better the performance of the model. Specifically, when AUC=0.5, the classification performance of the model is equivalent to random guessing; When AUC=1, the classification performance of the model is perfect. The calculation formula is:
    $$AUC = \frac{\sum_{i=1}^{M-1} (x_{i+1}-x_{i})\cdot(y_i+y_{i+1})}{2}$$

Where $M$ represents the total number of positive and negative samples, $x_i$represents FPR (false positive rate), $y_i$represents TPR (true case rate), which can be adjusted to obtain different FPRs and TPRs by adjusting the threshold value of the classification model. Each point on the ROC curve represents a different combination of FPR and TPR, and the AUC value is the size of the area under the ROC curve.\\
\\
\textbf{Mean Reciprocal Rank}  
Mean Reciprocal Rank (MRR) is an indicator used to measure the performance of ranking tasks (such as search, recommendation, etc.). It is the average reciprocal ranking of all queries. In information retrieval, MRR is often used to evaluate the quality of ranking results when a system answers a single query.

The MRR calculation method is to calculate the ranking of all documents returned by the system for each query. If a document matches the query, the reciprocal of its ranking is used as the score for the query, and the final score for all queries is averaged. The range of MRR values is 0 to 1. The higher the MRR value, the better the ranking of results the system can provide when answering queries.

The formula for MRR is as follows:

$$MRR = \frac{1}{|Q|}\sum_{i=1}^{|Q|}\frac{1}{rank_i}$$

Where $Q$ represents the query set, $|Q|$represents the total number of queries, and $rank_i$ indicates the ranking of the first correct document in the $i^{th}$ query. If the query does not have correct documents, then $rank_i$ Gets the total number of returned results from the query. The MRR value is the average of the reciprocal rankings of all queries.


==> content/sec7_old.tex <==
\section{Challenges}


\subsection{label sparsity}

Label sparsity, which pays more attention to the distribution of labels
situation, refers to that many labels in the label set are not assigned to any data sample, that is, there is a large gap between the label set and the sample set. Due to the scarcity of samples in some categories, the model is hard to capture the characteristics of these categories, which affects the final classification results. A challenge about label sparsity is that how to make better use of label information so that the model can learn the characteristics of all data samples. 

\subsection{label imbalance}

label imbalance refers to the situation that the number of training samples of different categories in the classification task varies greatly. Generally speaking, the model is easy to over-fit the categories with a large number, and under-fit the categories with a small number, so unbalanced training samples will lead the model to be more inclined to categories with more samples. Thus when a label appears only a few times, the classifier may choose to ignore it so that this category will not appear in the predicted results. The model will be more friendly to data with relatively balanced categories. So an urgent challenge is to consider how to balance the number of samples in different categories, so that the model can better handle the data of various categories. 

\subsection{label weak correlation}

In hierarchical multi-label classification task, label weak correlation means the weak correlation between labels at different levels or within the same level, that is, the dependency between labels is not obvious or difficult to capture. This will affect the classification results and performance of the model, thus what need to do is take corresponding measures to improve the correlation between labels. 

\subsection{low resource labeled data}

The lack of labeled data is still a big challenge. Although there are some methods, such as data enhancement, migration learning, unsupervised learning and semi-supervised learning, to reduce the use of labeled data, enough tag data is still needed to ensure the performance of the model and the accuracy of result is not particularly ideal. 

\subsection{Deep level prediction difficulty(low accuracy in deep level prediction)}

In hierarchical multi-label classification tasks, deep-level labels usually involve more specific concepts or categories, and these categories may appear less frequently in the data set, which makes it difficult for the model to extract deep features, resulting in greater difficulty in predicting deep-level labels and a corresponding decline in accuracy. Besides, in the model of hierarchical multi-label classification, incorrect classification of a classifier at one level may affect the results of the whole classification. Error classification result information at one level will be propagated to the next level, which causes low accuracy in deep level prediction. 

\subsection{Computational performance}

Because a large number of complex network models are used, such as convolution neural network, recurrent neural network, graph structure and tree structure, there are a lot of parameters to learn, which causes much time and resources on training.Thus a more important thing is to simplify model. 

\subsection{extreme multiple labels}
The Extreme Multi-Label Text Classification (XMTC) is the problem of selecting labels for one text from a collection of tens of thousands of labels. The difficulty of this task lies in the construction of the classifier, data sparsity caused by the long-tail distribution, difficulty in learning dependence patterns among labels, etc. The key of solving the problem is how to construct a classifier to solve the problem rather than building a classifier for each label group. We cannot directly group hierarchical labels because of the long- tail nature of XMC labels that lacks many positive samples of tags, nor can we crop tag sets, which makes tag dependency more difficult to capture.The common methods that XMTC handles are one VS all (OVA), embedding-based, and partitioning methods. Through these methods, a large number of XMC labels are divided into label groups and converted into multiple groups of simple label classification problems. The current common methods are: coding labels as a vector (Chalkidis et al., 2019) and labeling them individually (Gibaja, 2015). However, the effect is mediocre, because the former ignores the tag dependence and semantic information, while the latter can only be annotated partially.

==> content/sec8_old.tex <==
\section{Conclusions and Future Work}

In this article, we summarize several methods for dealing with hierarchical multi label classification problems. We divided the model into four major categories, summarized the dataset and evaluation indicators, and proposed the challenges faced by hierarchical multi label tasks.\\
\\Through research on model classification, it can be seen that early hierarchical multi label classification was based on a tree structure, with the parent label serving as the root node of the tree or subtree, and the child label serving as the leaf node of the tree or subtree. During classification, the prediction starts from the root node, and the prediction of related node labels is performed layer by layer according to the tree structure, until the leaf node. Modeling using tree structures is relatively complex and computationally expensive, so after the continuous development of deep learning, especially the introduction of transformer and bert, the method of using trees has gradually withdrawn from the stage. The current mainstream model is a serial model. Most models now divide the model into different levels based on the hierarchical structure of labels. For each level, a classifier can be set to classify labels, or information can be collected at each level. Finally, a global classifier is used to uniformly predict all labels. In engineering, there are also methods that use ensemble, which classify each category separately, and then talk about information fusion. However, this method is relatively rare in the field of scientific research. Another method is to input hierarchical structure information into the model as known information. Generally speaking, hierarchical structure is modeled through a graph model. When making predictions, the model can use the input hierarchical structure information to make predictions.\\
\\In the future, how to design a good classifier is a research direction. A good classifier can make good use of the relationship between text and layers of labels, as well as the dependency relationship between layers of labels. Secondly, finding a more suitable text encoding method can be regarded as a research direction, and whether there is a better text encoding method that can enable the network to better understand the information within the text. At the same time, as research continues to deepen, the problem of extreme multi label classification will become increasingly prominent, and the problem of long tailed data distribution will become increasingly prominent. Therefore, how to solve these two issues is also one of the future research directions.
